Enhancement of maximum superconducting temperature by applying pressure and reducing the charge transfer gap

Recent Scanning Tunneling Spectra(STS) measurement on underdoped cuprate discovers the increase of the maximum superconducting transition temperature $T_c$ when the size of charge transfer gap (CTG) is reduced. Applying pressure is another well known method to increase maximum $T_c$. However, these pressure experiments also found another puzzle that $T_c$ is enhanced in underdoped and optimal doped samples but suppressed in overdoped. Here we present a possible mechanism based on the charge fluctuation to explain both these two effects simultaneously. Starting from 3-band Hubbard model, we retrieve the charge fluctuation(CF) between oxygen 2$p^6$ band and copper 3$d^{10}$ band which is ignored in the $t-J$ model. This model is studied via variational Monte Carlo method(VMC).

==> conclusion.tex <==
In summary, based on experiment motivation, we include the CF into t-J model.  
The inclusion of charge transfer fluctuation enhance maximum pairing, presumably, maximum $T_c$. 
The decrease of charge transfer gap will increase Tc maximum but up to a limit. The fundamental reason of the extrema is because of finite value of of spinon density. The $\Delta_{var}$ would increase with spinon density while the renormalization factor $g_t$ decrease.	
However, in the overdoped side the CF will suppress pairing.
